PrIC3: Property Directed Reachability for MDPs

IC3 has been a leap forward in symbolic model checking. This paper proposes PrIC3 (pronounced pricy-three), a conservative extension of IC3 to symbolic model checking of MDPs. Our main focus is to develop the theory underlying PrIC3. Alongside, we present a first implementation of PrIC3 including the key ingredients from IC3 such as generalization, repushing, and propagation.

==> Makefile <==
.PHONY: default clean distclean


default: paper.pdf


.PHONY paper.pdf: *.tex literature.bib ./figures/*.tex ./algorithms/*.tex
	pdflatex -halt-on-error main && \
	cp main.pdf paper.pdf && \
	rm main.pdf

all: 
	pdflatex -halt-on-error main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main && \
	cp main.pdf paper.pdf && \
	rm main.pdf

spellcheck:
	for f in *.tex; do aspell check $$f; done

clean:
	rm -f *.aux *.log *.bbl *.blg *~ main.pdf *.out *.synctex.gz *.bak

distclean: clean
	rm -f main.pdf paper.pdf


==> algorithms/algorithm_check_refute.tex <==
% !TEX root = ../main.tex
%
\begin{figure}[t]
\begin{algorithm}[H]
%\setstretch{2}

%
 $\vars = \left\{ x_s ~\mid~s \in \ostates \right\}$ \tcp*{Notice that $\sinit \in \ostates$} 
 Let $\varphi$ be the following conjunction of inequalites:
 \textcolor{red}{Note: $\succs$ must include bad states! $G$ must be bad!}
 \[
    x_{\sinit} \leq  \lambda ~\wedge~
    \bigwedge_{s \in \ostates} ~ \bigwedge_{a \in \acts{s}}  x_s \geq \sum_{s' \in \succs (s)} P(s,a,s') \cdot 
    \begin{cases}
    x_{s'}, & \text{if}~s' \in \ostates \\
    1, & \text{if}~s' \in G  \\
    0, & \text{othwerise}
    \end{cases}~.
 \]
 %
 \uIf{$\varphi$ is unsatisfiable
 }{
	   \tcc{Property does not hold.}
      \Return $\true, \, \ostates$\;
 }
\uElse{
	  \Return $\false, \, \ostates$\;
}


    \caption{$ \checkrefutation \left( \thresh, \, \ostates \right)$}
\end{algorithm}
\end{figure}
%
%
%
%




==> algorithms/algorithm_get_probabilities.tex <==
%
\begin{figure}[t]

\begin{algorithm}[H]
%\setstretch{2}
    $\{s_1, \ldots, s_n\} \leftarrow \succs (s, a)$\;
    %
    %
    Let $\vars = \left\{ x_1, \ldots, x_n \right\}$\;
    %
    \uIf{$\oracle \left( x_1 \right) + \ldots +\oracle \left( x_n \right) \neq 0$}{
    Let $\varphi$ be the optimization problem
    %
    \begin{alignat}{2}
    %
       &\text{minimize} \qquad&&\sum_{\substack{x_i \in \vars \\  s_i \not \in \bad}} \abs{\frac{x_i}{x_1+\ldots+x_n} - \frac{\oracle \left( x_i \right)}{\oracle \left( x_1 \right) + \ldots +\oracle \left( x_n \right)}} \notag \\
       %
       &\text{s.t.} &&\phantom{\eewedge} \delta \eeq \sum_{x_i \in \vars} P(s, a , s_i) \cdot 
       \begin{cases}
       1, & \text{if}~s_i \in \bad \\
       x_i, & \text{if}~\text{otherwise}
       \end{cases} \notag \\
       %
       &&&\eewedge   \bigwedge_{\substack{x_i \in \vars  \\ s_i \in \cstates}} x_i = F[s_i]  \quad  \eewedge \quad \bigwedge_{x_i \in \vars} 0 \leq x_i \leq 1~. \notag
    %
    \end{alignat}
    }
    %
    \uElse{
    	%
    	\tcc{All oracle values are $0$. Break down probability mass equally.}
       %
       Let $\varphi$ be the equation system
       %
       \begin{align*}
          &  \delta \eeq \sum_{x_i \in \vars} P(s, a, s_i) \cdot 
          \begin{cases}
          1, & \text{if}~s_i \in \bad \\
          x_i, & \text{if}~\text{otherwise}
          \end{cases} \\
          %
        \wedge   & \bigwedge_{\substack{
        	i,j \in \{1,\ldots,n \} \\
        	i < j \\
        	s_i, s_j \not \in \cstates
        }}  x_i = x_j 
    \quad
    %
    \wedge 
    %
    \quad
    %
   \bigwedge_{\substack{x_i \in \vars  \\ s_i \in \cstates}} x_i = F[s_i]
    %
    \quad
    %
    \wedge
    %
    \quad
    %
     \bigwedge_{x_i \in \vars} 0 \leq x_i \leq 1~.
       \end{align*}
       %
       %
       %
    }
    %
    \uIf{ $\varphi$ has a solution $\sol \in [0,1]^{\vars}$}
    {
       \Return $\true,  \, \sol \left[ x_1 \right], \ldots, \sol \left[ x_n \right]$\;
    }
    \uElse{
		\Return $\false$\;
}
	%
	%
    \caption{$ \getprobs \left( s, \, a, \, \delta, \,  F, \,  \oracle , \, \cstates \right)$}
\end{algorithm}
%
\kevin{Require $a \in \acts{s}$?}
\end{figure}
%
%
%
%




==> algorithms/algorithm_refine_oracle.tex <==
%
\begin{figure}[t]
\begin{algorithm}[H]
%\setstretch{2}
 \uIf{$\vstates \subseteq \ostates$}
 {
  \tcc{Adding $\vstates$ to $\ostates$ does not yield progress. We thus ensure progress by:}
  $\ostates \leftarrow \ostates \cup \big( \succs($\ostates$)  \setminus G \big)$\;
 }
 \uElse
 {
   $\ostates \leftarrow \ostates \cup \vstates$\;
 }
 %
 $\vars = \left\{ x_s ~\mid~s \in \ostates \right\}$\;
 Let $\sol \in \textcolor{orange}{\realsgeqz}^\vars$ be the solution of the following linear program:
 %
 %
 \begin{alignat*}{2}
  &\text{minimize} \qquad &&x_{\sinit} \\
  %
    &\text{s.\ t.\ } &&\bigwedge_{s \in \ostates } \, x_s \geq 0 \, \wedge \, \bigwedge_{a \in \acts{s}} x_s \geq  \sum_{s' \in \textnormal{Succs(s)}} P(s, a, s') \cdot 
    \begin{cases}
    x_{s'}, & \text{if}~s' \in \ostates \\
    1, & \text{if}~s' \in G  \\
    \oracle(s'), & \text{othwerise}
    \end{cases} ~.
 \end{alignat*}
 %
 \For{$s \in \ostates$}{
 	$\oracle[s] \leftarrow \sol[x_s]$\;
 } 
 %
 \Return $\oracle, \, \ostates$\;

    \caption{$ \refineoracle \left( \vstates, \, \ostates, \, \oracle \right)$}
\end{algorithm}

\end{figure}
%
%
%
%




==> algorithms/algorithm_strenghten.tex <==
\begin{figure}[p]
\begin{algorithm}[H]
%\setstretch{2}
 \KwData{\quad MDP $\mdp$,\quad bad states $\bad$,\quad  threshold $\lambda$,\quad \changed{oracle} $\changed{\oracle \in \textcolor{red}{\realsgeqz}^{\sqm}}$}
 \KwResult{\quad $\unsafe$ and a subsystem if the MDP is unsafe or $\oracle$ is insufficent; $\safe$ otherwise}
\SetNoFillComment
%
 %
$Q \leftarrow \{(k, \sinit, \textcolor{red}{\lambda})\}$ \;
%
%
\While{$Q$ not empty}{
   $(i, s, \textcolor{red}{\delta}) \leftarrow Q.\qpop$ \; 
   \tcc{Pop obligation with smallest frame index $i$. Meaning: Make update $F_i[s] \leftarrow \textcolor{red}{\delta}$ possible, i.e., prove that
   $\prevtbmax{\mdp}{s}{i}{\bad} \leq \textcolor{red}{\delta}.$}
   %
   $\textcolor{red}{\vstates \leftarrow \vstates \cup \{s\}}$\;
   %
   \uIf{$i = 0$}{
           \tcc{\textcolor{red}{possible} counterexample given by subsystem consisting of states popped from Q at some point}
           \Return $\false$\textcolor{red}{, $\hdots$, Q.touchedStates()};
           %\textcolor{red}{ \Throw new PossiblyUnsafe(Q.history(s))}
           %\textcolor{red}{\Return \checkrefutation\left( \thresh, $\textcolor{red}{
      $\textcolor{red}{\oracle, \, \ostates \leftarrow \refineoracle \left( \vstates, \, \ostates, \, \oracle \right)}$\;
      %\uIf{$\refute$}
      %{
      %  \Return $\true$\;
     %}
      %
      $\refute \leftarrow \checkrefutation \left( \thresh, \, \ostates\right)$\;
      %
      \uIf{$\refute$}{
         \Return $\true, \, F_0,\ldots,F_k, \, \textcolor{red}{\oracle}$\;
      }
      \uElse{
         $\textcolor{red}{\vstates \leftarrow \emptyset}$\;
         $Q \leftarrow \{(k, \sinit,\textcolor{red}{ \thresh})\}$\;
      }
   }
   \uElse{
      \uIf(for such an $a$){$\exists a \in \acts{s} \colon \bma{a}{F_{i-1}}[s] > \textcolor{red}{\delta}$}{
      	%
      	\tcc{
      		Since $\acts{s}$ is finite, we check a finite disjunction here.
      	}
      	%
      	%
      \tcc{The update $F_i[s] \leftarrow \textcolor{red}{\delta}$ would violate relative inductiveness. Refine $F_{i-1}$.}
      %
      %
          $\{s_1, \ldots, s_n\} \leftarrow \succs(s, a)$\tcc*{might be extracted from SMT query}
          %
          %
          $\textcolor{red}{\success, \delta_1,\ldots,\delta_n \leftarrow \getprobs\left( s, \, a, \, \delta, \,  F_{i-1} ,  \, \oracle , \, \vstates \right)}$ \;
          %
          %
          \uIf{\textcolor{red}{$\success$}}{
             $Q.\qpush{\left(i-1, s_1,  \textcolor{red}{\delta_1} \right), \ldots, \left(i-1, s_n,  \textcolor{red}{\delta_n} \right)}$\;
             %
             $Q.\qpush{ \left( i, s, \delta \right) }$\;
          }
      %
         \textcolor{red}{
          \uElse{
             $\textcolor{red}{\oracle, \ostates \leftarrow \refineoracle \left( \vstates, \, \ostates, \,  \oracle \right)}$\;
             $\refute \leftarrow \checkrefutation \left( \thresh, \, \ostates \right)$\;
             %
      \uIf{$\refute$}{
         \Return $\true, F_0,\ldots,F_k, \textcolor{red}{\oracle}$\;
      }
      \uElse{
         $\textcolor{red}{\vstates \leftarrow \emptyset}$\;
         $Q \leftarrow \{(k, \sinit,\textcolor{red}{ \thresh})\}$ \;
      }
          }
          }
      %
      }
      \uElse
      {
       \tcc{The update $F_i[s] \leftarrow \textcolor{red}{ \delta}$ does \emph{not} violate relative inductiveness. Update frames and reenqueue..}
       %
       %
       \uIf{$i < k $}{
       	%
           $Q.\qpush{\left( i+1, s, \textcolor{red}{\delta}  \right) }$\;
       %
       }
       %
       \uIf{$ i + 1 \neq k$}{
	   %
          $\textcolor{red}{\vstates \leftarrow \vstates \setminus \left\{s\right\}}$\;
       }
       %
       \kevin{generalize here}
       %
         $F_1[s] \leftarrow \minval{F_1[s], \, \textcolor{red}{\delta}}; \ldots ; F_i[s]  \leftarrow \minval{F_i[s], \, \textcolor{red}{\delta}}$\;
         %
        $ \textcolor{red}{\vstates \leftarrow \vstates \setminus \{ s \}}$\;
      }
   }
}
%
%
   \Return $\false, \, F_0,\ldots ,F_k, \, \textcolor{red}{\oracle, \, \ostates}$\;
   
   \caption{$\strengthencall{F_0, \ldots,F_k}{\textcolor{red}{\oracle}}{\textcolor{red}{\ostates}}$}
\end{algorithm}
\end{figure}


==> algorithms/strengthen_parttwo.tex <==
\begin{figure}[t]
\begin{algorithm}[H]
%\setstretch{2}
\SetNoFillComment
%

   %
   \uIf{lost obligation}{
   $\refute \leftarrow \checkrefutation \left( \thresh, \, \ostates\right)$\;
      %
      \lIf{$\refute$}{
         \Return $\true, \, F_0,\ldots,F_k, \, \textcolor{red}{\oracle}$
      }
      \uElse{

      $\textcolor{red}{\oracle, \, \ostates \leftarrow \refineoracle \left( \vstates, \, \ostates, \, \oracle \right)}$\;
      
         $\textcolor{red}{\vstates \leftarrow \emptyset}$\;
         $Q \leftarrow \{(k, \sinit,\textcolor{red}{ \thresh})\}$\;
      }
   }
      \caption{$\strengthencall{F_0, \ldots,F_k}{\textcolor{red}{\oracle}}{\textcolor{red}{\ostates}}$}
\label{alg:loststrengthen}
\end{algorithm}
\end{figure}

==> bib.tex <==
\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}

==> detailed-code.tex <==

\input{algorithms/algorithm_get_probabilities}


\input{algorithms/algorithm_check_refute}

\input{algorithms/algorithm_refine_oracle}

==> figures/bad-chain.tex <==
\begin{tikzpicture}[every node/.style={font={\scriptsize}}, shorten >=1pt,nodestyle/.style={draw,circle,font={\scriptsize}},actstyle/.style={draw,circle,fill=black,inner sep=1pt}]


	\node[nodestyle,initial text=, initial where=left] (s0) {$s_0$};
    \node[above=0.3cm of s0] (init) {};
	\node[nodestyle,left=1cm of s0] (s1) {$s_1$};
	\node[nodestyle,left=1cm of s1] (s2) {$s_2$};
	\node[nodestyle,right=1cm of s0] (s3) {$s_3$};
	\node[nodestyle,right=1cm of s3] (s4) {$s_{4}$};
    \node[nodestyle,fill=Crimson,right=1cm of s4] (s5) {$\textcolor{white}{s_{5}}$};
			
			
	\draw[->] (init) edge (s0);
	\draw[->] (s0) edge node[above] {$\sfrac 1 2$} (s1);
	\draw[->] (s0) edge node[above] {$\sfrac 1 2$} (s3);
    \draw[->] (s1) edge node[above] {$1$} (s2);
    \draw[->] (s2) edge[loop left] node[left] {$1$} (s2);
	\draw[->] (s3) edge node[above] {$1$} (s4);
	\draw[->] (s4) edge node[above] {$1$} (s5);
    \draw[->] (s5) edge[loop right] node[right] {$1$} (s5);

\end{tikzpicture}


==> figures/chain.tex <==

\begin{tikzpicture}[every node/.style={font={\scriptsize}}, shorten >=1pt,nodestyle/.style={draw,circle,font={\scriptsize}},actstyle/.style={draw,circle,fill=black,inner sep=1pt}]


	\node[nodestyle, initial, initial text=, initial where=left] (s0) {$s_0$};
	\node[nodestyle,right=1cm of s0] (s1) {$s_1$};
	\node[nodestyle,right=1cm of s1] (s2) {$s_2$};
	\node[right=1cm of s2] (s3) {$\ldots$};
	\node[nodestyle,right=1cm of s3] (s4) {$s_{N-2}$};
	\node[nodestyle,right=1cm of s4] (s5) {$s_{N-1}$};
	\node[nodestyle,right=1cm of s5] (s6) {$s_{N}$};
			
			
		\node[nodestyle, below=1cm of s0] (b0) {$b_0$};
		\node[nodestyle,right=1cm of b0] (b1) {$b_1$};
		\node[nodestyle,right=1cm of b1] (b2) {$b_2$};
		\node[right=1cm of b2] (b3) {$\ldots$};
		\node[nodestyle,right=1cm of b3] (b4) {$b_{N-2}$};
		\node[nodestyle,right=1cm of b4] (b5) {$b_{N-1}$};
	
	\draw[->] (s0) edge node[above] {$p$} (s1);
		\draw[->] (s1) edge node[above] {$p$} (s2);
	\draw[->] (s2) edge node[above] {$p$} (s3);
	\draw[->] (s3) edge node[above] {$p$} (s4);
	\draw[->] (s4) edge node[above] {$p$} (s5);
	\draw[->] (s5) edge node[above] {$p$} (s6);

    \path[->] (s0) edge node[left] {$1-p$} (b0);
		\draw[->] (s1) edge node[left] {$1-p$} (b1);
			\draw[->] (s2) edge node[left] {$1-p$} (b2);

							\draw[->] (s4) edge node[left] {$1-p$} (b4);
									\draw[->] (s5) edge node[left] {$1-p$} (b5);
	
	
	%\draw[->] (s0) edge node[above] {$\nicefrac{1}{2}$} (s2);
	
	%\draw[-] (s2) -- node[above] {$a$} (a); 
	%\draw[-] (s2) --  node[right] {$b$} (b); 
	
	%\draw[->] (b) edge[bend left=20] node[above] {$1$} (s0);

	%\draw[->] (s1) edge[bend left=20] node[above] {$\nicefrac{1}{2}$} %(s0);
	%\draw[->] (s1) edge node[above] {$\nicefrac{1}{2}$} (s3);
	
	%\draw[->] (s3) edge[bend right=30] node[above, pos=0.2] %{$\nicefrac{1}{3}$} (s4);
	%\draw[->] (s3) edge node[above] {$\nicefrac{2}{3}$} (s5);
	%\draw[->] (a) edge node[above] {$\nicefrac{1}{2}$} (s4);
	%\draw[->] (a) edge[bend right=15] node[above] {$\nicefrac{1}{2}$} %(s5);

	
	%\draw[->] (s4) edge[loop left] node[left] {$1$} (s4);
	%\draw[->] (s5) edge[loop right] node[right] {$1$} (s5);
\end{tikzpicture}


==> figures/double_chain.tex <==

\begin{tikzpicture}[every node/.style={font={\scriptsize}}, shorten >=1pt,nodestyle/.style={draw,circle,font={\scriptsize}},actstyle/.style={draw,circle,fill=black,inner sep=1pt}]


	
	
	
	
	





	\node[nodestyle, initial, initial text=, initial where=left] (s0) {$s_0$};
	\node[nodestyle,right=1cm of s0] (s1) {$s_1$};
	\node[nodestyle,right=1cm of s1] (s2) {$s_2$};
	\node[right=1cm of s2] (s3) {$\ldots$};
	\node[nodestyle,right=1cm of s3] (s4) {$s_{N-2}$};
	\node[nodestyle,right=1cm of s4] (s5) {$s_{N-1}$};
	\node[nodestyle,right=1cm of s5] (s6) {$s_{N}$};
			
			
		\node[nodestyle, below=1cm of s0] (b0) {$b_0$};
		\node[nodestyle,right=1cm of b0] (b1) {$b_1$};
		\node[nodestyle,right=1cm of b1] (b2) {$b_2$};
		\node[right=1cm of b2] (b3) {$\ldots$};
		\node[nodestyle,right=1cm of b3] (b4) {$b_{N-2}$};
		\node[nodestyle,right=1cm of b4] (b5) {$b_{N-1}$};
	
	\draw[->] (s0) edge node[above] {$p$} (s1);
		\draw[->] (s1) edge node[above] {$p$} (s2);
	\draw[->] (s2) edge node[above] {$p$} (s3);
	\draw[->] (s3) edge node[above] {$p$} (s4);
	\draw[->] (s4) edge node[above] {$p$} (s5);
	\draw[->] (s5) edge node[above] {$p$} (s6);
	
		\draw[->] (s0) edge node[left] {$1-p$} (b0);
		\draw[->] (s1) edge node[left] {$1-p$} (b1);
			\draw[->] (s2) edge node[left] {$1-p$} (b2);

							\draw[->] (s4) edge node[left] {$1-p$} (b4);
									\draw[->] (s5) edge node[left] {$1-p$} (b5);
	
	
	%\draw[->] (s0) edge node[above] {$\nicefrac{1}{2}$} (s2);
	
	%\draw[-] (s2) -- node[above] {$a$} (a); 
	%\draw[-] (s2) --  node[right] {$b$} (b); 
	
	%\draw[->] (b) edge[bend left=20] node[above] {$1$} (s0);

	%\draw[->] (s1) edge[bend left=20] node[above] {$\nicefrac{1}{2}$} %(s0);
	%\draw[->] (s1) edge node[above] {$\nicefrac{1}{2}$} (s3);
	
	%\draw[->] (s3) edge[bend right=30] node[above, pos=0.2] %{$\nicefrac{1}{3}$} (s4);
	%\draw[->] (s3) edge node[above] {$\nicefrac{2}{3}$} (s5);
	%\draw[->] (a) edge node[above] {$\nicefrac{1}{2}$} (s4);
	%\draw[->] (a) edge[bend right=15] node[above] {$\nicefrac{1}{2}$} %(s5);

	
	%\draw[->] (s4) edge[loop left] node[left] {$1$} (s4);
	%\draw[->] (s5) edge[loop right] node[right] {$1$} (s5);
\end{tikzpicture}


==> fullexample.tex <==
\begin{figure}
\subfloat[]{
\begin{tabular}{l|c|cc|ccc}
Iteration & 1                & \multicolumn{2}{c|}{2}                  & \multicolumn{3}{c}{3}                                              \\
Frame     & 1                & 1                   & 2                 & 1                   & 2                   & 3                 \\\hline
$s_0$     & $\nicefrac{5}{9}$ & $\nicefrac{5}{9}$    & $\nicefrac{5}{9}$  & $\nicefrac{5}{9}$    & $\nicefrac{5}{9}$    & $\nicefrac{5}{9}$  \\
$s_1$     & $1$              & $\nicefrac{11}{18}$ & $1$               & $\nicefrac{11}{18}$ & $\nicefrac{11}{18}$ &  $1$                 \\
$s_2$     & $1$              & $\nicefrac{1}{2}$   & $\nicefrac{1}{2}$ & $\nicefrac{1}{2}$   & $\nicefrac{1}{2}$   & $\nicefrac{1}{2}$ \\
$s_3$     & $1$              & $1$                 & $1$               & $\nicefrac{2}{3}$   & $\nicefrac{2}{3}$   &  $1$                
\end{tabular}
}
\subfloat[]{
}	
\caption{The same invocation as in ..., but with propagation and repushing enabled.}
\end{figure}

==> outdated/encoding.tex <==

%\textbf{Objects}:
%
%\begin{itemize}
	%\item For every smt-int/smt-bool variable, we have a prism-int/prism-bool variable: $\varc$ and $\varf$.
	%
	%\item We have an uninterpreted function $\fun{\Frame}{\Ints}{\Reals}$ representing the frame.
   %            Interpretation:
	%           Let $\valc \in \{ 0,\ldots,20 \}$ and let $F$ be the frame represented by the solver instance. If $\Frameapp{\valc}{\valf} = d$ is a (partial) satisfying model, then $F[\valc, \valf]\geq d$.  
	%
	%
	%\item We have an uninterpreted function $\fun{\smtbm}{\Ints}{\Reals}$ representing the Bellman operator.  Interpretation:
%	Let $\valc \in \{ 0,\ldots,20 \}$ and let $F$ be the frame represented by the solver instance. If $\smtbmapp{\valc}{\valf} = d$ is a (partial) satisfying model, then $\bm{F}[ \valc, \valf ] \geq d$.  
	%
	%
	%\item We have a predicate $\fun{\Goal}{\Ints \times \Bools}{\Bools}$ such that
	  %         $\Goalapp{\valc}{\valf}$ iff $(\valc, \valf)$ is a goal state.	
	%
	%\item We have an smt-int $\chosencmd$ representing command-indices.
%\end{itemize}

%\textbf{Permanent assertions}:
%
%\begin{itemize}
%	\item Assert that all integer variables are in the range defined by the program: $0 \leq \varc \leq 20$.
	%
%	\item Assert that $\chosencmd$ evaluates to a command index: $\chosencmd \in \{ 0 , 1 \}$.
	%
%	\item Define $\Goal$:
	%
%	\[ \niceforall \valc, \valf \colon \Goalapp{\valc}{\valf} \Leftrightarrow \valf = \true ~.\]
	%
	%\item Assert that the frame evaluates to at most $1$:
%		\[ \niceforall \valc, \valf \colon \Frameapp{\valc}{\valf} \leq 1 ~. \]
	%
%	\item Define (a sufficient subset of) $\szero$ as the set of states that are no goal state and where no command is active (in case the program does not terminate almost--surely, then this subset does not suffice to prove every upper bound).:
	%
%	\begin{align*}
	%    & \niceforall \valc, \valf \colon \neg \Goalapp{\valc}{\valf} \wedge \neg (\valc < 20) \wedge \neg (\valc < 10) \\
	    %
	%     &\quad \quad \quad  \quad \quad \quad \quad         \Longrightarrow
	    %       \left( \Frameapp{\valc}{\valf} = 0 \wedge \smtbmapp{\valc}{\valf} = 0  \right)
	%\end{align*}
	%
	%\item Assert that bellman-of-goal-state is $1$:
	%
	%\[
	%   \niceforall \valc, \valf \colon \Goalapp{\valc}{\valf}
%	   \Longrightarrow \smtbmapp{\valc}{\valf} = 1
	%\]
	%
	%\item Assert that if some of the commands is active, then one of the active commands must be chosen by $\chosencmd$:
	%
	%\begin{align*}
	%   &\left( \varc \leq 20 \vee \varc \leq 10 \right) \\
	   %
	%    &\qquad \Longrightarrow \left(  (\varc \leq 20 \wedge \chosencmd = 1)  \vee (\varc \leq 10 \wedge \chosencmd = 2) \right)
	%\end{align*}
	%
	\item Finally, encode the result of the bellman operator for each command. Note that 
	          we execute a command only if it is no goal state.
	          \kevinmargin{@Sebastian: Does this encoding enforce that ChosenCommand really corresponds to the command that is responsible for the non-relative-inductivenss in case of a SAT call?
	           The quantifier confuse me right now..}
	%
	\begin{enumerate}
		%
		  \item 
		   %
		   \begin{align*}
		         &\niceforall \valc, \valf \colon \neg \Goalapp{\valc}{\valf} \wedge 
		             \valc \leq 20 \wedge \chosencmd = 1  \\
		             %
		             %
		            & \quad  \Longrightarrow
		          \smtbmapp{\valc}{\valf} = 0.1 \cdot \Frameapp{\valc}{\true} + 0.9 \cdot \Frameapp{\valc + 1 }{\valf}
		   \end{align*}
		%
		%
		\item 
		%
		\begin{align*}
			&\niceforall \valc, \valf \colon \neg \Goalapp{\valc}{\valf} \wedge 
			\valc \leq 10 \wedge \chosencmd = 2 \\
			%
			%
			& \quad  \Longrightarrow
			\smtbmapp{\valc}{\valf} = 0.05 \cdot \Frameapp{\valc}{\true} + 0.95 \cdot \Frameapp{\valc + 2 }{\valf}
		\end{align*}
	\end{enumerate}
	
\end{itemize}

%
%\textbf{Strengthening of Frames:}
%%
%\begin{itemize}
%	\item Ungeneralized constraint: $\Frameapp{2,0} \leq \nicefrac{1}{2}$.
%	\end{itemize}
%
%%
%\textbf{Queries:}
%%
%\begin{itemize}
%	\item Relative inductiveness query for ungeneralized constraints: 
%	%
%	\[ \varc = 2 \wedge \varf = \false \wedge \smtbmapp{\varc}{\varf} > \nicefrac{1}{2} ~. \]
%	%
	
%\end{itemize}

%	\item We apply a ``clever" kind of Ackermann reduction to avoid uninterpreted functions. 
	%
	%\item We avoid quantifiers at the cost of an encoding whose number of constraints grows linearly in the number of \emph{updates} in the program (the example program above has $4$ updates). For our example, pushing a constraint of the form $\Frameapp{2}{\false} \leq \nicefrac{1}{2}$
	%requires pushing $4$ constraints.
	%
%	\item Without generalization (or at most linear generalization), we are thus in the theory of Linear Integer Arithmetic (QFNIA).
	%





==> partial_correctness.tex <==
%
%
%
This subsection is devoted to showing the following theorem. \sebastian{shouldn't we formulate it such that partial correctness including generalization is handled... i.e., put generalization (and maybe repushing) somewhere before?}
\begin{theorem}
\label{thm:strenghtencorrect}
   Procedure $\strengthen$ satisfies its specification.
\end{theorem}	
As a straightforward consequence of Theorems~\ref{thm:strengthencorrecticcorrect} and~\ref{thm:strenghtencorrect} we obtain:
\begin{theorem}
\label{thm:priccorrect}
   Procedure $\prict$ satisfies its specification.
\end{theorem}

%%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%

==> proof_pric3correct.tex <==
For expressing partial correctness of \pricthree as Hoare triples, we will reformulate both $\prevtmax{\mc}{\sinit}{\bad} \leq \thresh$ and $\prevtmax{\mc}{\sinit}{\bad} > \thresh$ in a way which is closer to our way of thinking in terms of frames.
Namely, because of continuity of $\bmsymbol$, we have 
%
\begin{align*}
	\prevtmax{\mc}{\sinit}{\bad} \lleq \thresh &\qqiff \forall\, n \colon \quad \bmnapp{n}{\zeroexp}{\sinit} \lleq  \thresh~, \qquad\quad \text{and} \\
	\prevtmax{\mc}{\sinit}{\bad} \GG \thresh &\qqiff \exists\, n \colon \quad \bmnapp{n}{\zeroexp}{\sinit} \GG  \thresh~.
\end{align*}%
%
%


Formally, we have the following specification.
%
%
Our partial correctness specification for \pricthree hence reads as follows:
%
%
\begin{definition}[Specification of $\boldpricthree$]
\label{def:spec_pric3}
	\pricthree is partially correct if the following two Hoare triples are valid:
	%
	\begin{align*}
		1.~ \htriple{\forall\, n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq  \thresh}
				{\prictcall{\mdp}{\bad}{\thresh}{\oracle}}
				{\return =  \safe} \phantom{\texttt{UN}} \\[.5em]
		%
		2.~\htriple{\exists\, n \colon \bmnapp{n}{\zeroexp}{\sinit} >  \thresh}
				{\prictcall{\mdp}{\bad}{\thresh}{\oracle}}
				{\return =  \unsafe}
		%
		\tag*{$\triangle$}                 
	\end{align*}%
	%
\end{definition}

\begin{definition}[Specification of $\propagate$]
\label{def:spec_propagate}
	%
	\propagate is partially correct if the following Hoare triple is valid:
	%
		%
		\begin{align*} 
		%
		& \big\{ \icinv{F_0,\ldots,F_{k}} \eewedge F_k \leq F_{k+1} \eewedge \bm{F_k} \leq F_{k+1}  \big\}\\[0.4em]
		%
		& \quad F_0, \ldots,F_{k+1} \lleftarrow \propagatecall{F_0, \ldots, F_{k+1}} \\[0.4em]
		%
		& \big\{ \icinv{F_0,\ldots,F_{k}} \eewedge F_k \leq F_{k+1} \eewedge \bm{F_k} \leq F_{k+1}   \big \}
		%
		\end{align*}
        %
	%
\end{definition}%

\begin{proof}
	We consider the cases $\prevmax{\bad} \leq \thresh$ and  $\prevmax{\bad} > \thresh$ separately. \\ \\
	%
	\noindent
	\emph{The case $\prevmax{\bad} \leq \thresh$.} Assume $\forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh$. We show that if $\prictcall{\mdp}{\bad}{\thresh}{\oracle}$ terminates,
	then $\return = \safe$. Towards this end, we propose the following loop invariant $I$ for the loop beginning in line~$\lineprictloopstarts$:
	%
	\begin{align*}
	    I \eeq&  \forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh \eewedge \icinv{F_0,\ldots,F_{k-1}} \eewedge F_{k-1} \leq F_k \eewedge \bm{F_{k-1}} \leq F_k 
	\end{align*}
	%
	%
	%
	We now verify that the loop invariant holds at the beginning of the loop (initialization) and that it is preserved by each iteration (consecution).
	Notice that $ \forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \lambda$ holds at all times since no input except for the oracle $\oracle$ is altered during execution.  \\ \\
	%
	\noindent
	\textbf{Initialization.} The condition $\forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq  \thresh$ holds by assumption. After lines $1$--$4$, we have $k=1$, $F_0 = \zeroexp$, and $F_1 = \oneexp$. We have
	%
	\begin{align*}
	   &\icinv{F_0, \ldots F_{k-1}} \\
	   %
	   \textnormal{iff}\qquad&\icinv{F_0} \\
	   %
	   \textnormal{iff}\qquad&F_0 = \zeroexp \\
	   %
	   \textnormal{iff}\qquad& \true~.
    \end{align*}
    %
    %
    Moreover, $F_{k-1}= F_0 = \zeroexp \leq \oneexp = F_1 = F_k$
    and $\bm{F_{k-1}}\leq \oneexp = F_1 = F_k$ hold trivially.
	%
	Hence, $I$ holds at the beginning of the loop. \\ \\
	%
	\noindent
	\textbf{Consecution.} Assume the loop invariant $I$ holds at the beginning of some iteration. 
	This implies that the precondition of the specification in Definition~\ref{def:spec_strengthen}.1 is satisfied.
	Hence, on termination of the call $\strengthencall{F_0, \ldots,F_k}{\oracle }{\ostates}$, we have $\refute = \false$
	and $\icinv{F_0,\ldots, F_k}$. We thus do not enter the if-branch in line $5$ and initialize $F_{k+1} = \oneexp$. Hence, we satisfy the specification of $\propagate$ (Def.\ \ref{def:spec_propagate}) and the call to $\propagate$ in line $7$ preserves $ \icinv{F_0,\ldots,F_{k}} \wedge F_k \leq F_{k+1} \wedge \bm{F_k} \leq F_{k+1}$.  There are now two cases: Either the condition of the 
	if-statement in line $8$ evaluates to $\true$ and the loop terminates with $\return = \safe$, or we execute lines $9$.
	For the former case, we have nothing to show. For the latter case, i.e., executing line $9$, the loop invariant $I$ is reestablished.
	%
	\\ \\
	%
	Invariant $I$ implies that if the call $\strengthencall{F_0, \ldots,F_k}{\oracle }{\ostates}$ in line $4$ terminates, we have
	$\refute = \false$. Since the loop of $\prict$ can only terminate in line $5$ or in line $8$, termination of $\prict$ implies that $\return = \safe$. \\ \\
	%
	%
	\emph{The case $\prevmax{\bad} > \thresh$.} Assume $\exists n \colon \bmnapp{n}{\zeroexp}{\sinit} > \thresh$. We have to show that if $\prictcall{\mdp}{\bad}{\thresh}{\oracle}$ terminates, 	then we have $\return = \unsafe$. Towards this end, we propose the following loop invariant $I$ for the loop beginning in line $\lineprictloopstarts$:
	%
	\begin{align*}
	I \eeq& \exists n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh \eewedge \icinv{F_0,\ldots,F_{k-1}} \eewedge F_{k-1} \leq F_k \eewedge \bm{F_{k-1}} \leq F_k
	\end{align*}
	%
	As for the previous case, we proceed by verifying initialization and consecution. \\ \\
	%
	\noindent
	\textbf{Initialization.} This is analogous to the previous case since $\exists n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh$ holds at all times. \\ \\
	%
	%
	\noindent
	\textbf{Consecution.} Assume the loop invariant $I$ holds at the beginning of some iteration. 
	This implies that the precondition of the specification in Definition~\ref{def:spec_strengthen}.2 is satisfied.
	Hence, on termination of the call $\strengthencall{F_0, \ldots,F_k}{\oracle }{\ostates}$, we encounter exactly one of the following two cases:
	%
	\begin{alignat}{2}
		%
		\textnormal{Case 1:} \quad &
	    \refute =  \false \notag
	    \eewedge \icinv{F_0, \ldots, F_k}   \notag \\[0.3em]
	     %
	     %
	     \textnormal{Case 2:} \quad & \refute =  \true   \notag
	     %
	\end{alignat}
	%
	%
	\emph{Case 1.} Since $\refute = \false$, we do \emph{not} enter the if-branch in line $5$. The fact that $I$ is reestablished at the end of the iteration
	is thus completely analogous to the case $\prevmax{\bad} \leq \thresh$. \\ \\
	%
	%
	\emph{Case 2.} Since $\refute = \true$, we \emph{do} enter the if-branch in line $5$, which yields $\prict$ to terminate with $\return = \unsafe$.
	 Hence, we have nothing to show. \\ \\
	%
	%
	Our invariant $I$ now implies that if $\strengthencall{F_0, \ldots,F_k}{\oracle }{\ostates}$ in line $6$ terminates, we 
	either terminate with $\return = \unsafe$ or we have $\icinv{F_0,\ldots,F_k}$.  If  $\icinv{F_0,\ldots,F_k}$ holds, then, by the contraposition to Lemma~\ref{lem:ic3_inv_eqframes}, we have
	$\neg \eqframes{F_1,\ldots,F_k}$. Since the loop of $\prict$ can only terminate in line $5$ or in line $8$, termination of $\prict$ implies that $\return = \unsafe$.
	%
\end{proof}

==> proof_strengthen_correct.tex <==

\christoph{start \atkevin Perhaps you want to move the definition below somewhere else.}
For later reference, let us briefly recall the formal specification required of our heuristic \heuristic.
\begin{definition}[Specification of $\getprobs$]
	\label{def:spec_getprobs}
	%
	\kevinmargin{Adapt the specification such that in includes $\cstates$ or be more generic here?}
	\sebastianmargin{signature should match}
	%
	\begin{enumerate}
	%
	\item The case \emph{probabilities exist}: \label{def:spec_getprobs_exists}
		\begin{align*}
		&\big\{  \exists \bar{\delta} \in [0,1]^{|\succs(s,a)|} \colon \bma{a}{F \substleft \succs(s,a) \substarrow \bar{\delta} \substright }[s] \leq \delta  \big\} \\[0.4em]
		%
		&\quad \getprobs \left( s, a, \delta, F, S'\right) \\[0.4em]
		%
		&\big\{ \return = \true, \bar{\delta} \eewedge \bar{\delta} \in [0,1]^{|\succs(s,a)|}  
		\eewedge \bma{a}{F\substleft \succs(s,a) \substarrow \bar{\delta} \substright}[s] \leq \delta \big\}
		%
		\end{align*}
	%
	\item The case \emph{probabilities do not exist}: \label{def:spec_getprobs_not_exists}
	\begin{align*}
	&\big\{  \neg\exists \delta \in [0,1]^{|\succs(s,a)|} \colon \bma{a}{F \substleft \succs(s,a) \substarrow \bar{\delta} \substright }[s] \leq \delta \big\} \\[0.4em]
	%
	&\quad \getprobs \left( s, a, \delta, F, \oracle \right) \\[0.4em]
	%
	&\big\{ \return = \false, \ldots  \big\}
	%
	\end{align*}
	%
	%
	%
	\end{enumerate}
	%
	%
	
\end{definition}
\christoph{end}

    We consider the cases $\prevmax{\bad} \leq \thresh$ and  $\prevmax{\bad} > \thresh$ separately. \\ \\
	%
	\noindent
	\emph{The case $\prevmax{\bad} \leq \thresh$.} We have to show that if $\strengthencall{F_0, \ldots, F_k}{\oracle}{\ostates}$ terminates, then
	$\return = \false,F_0,\ldots, F_k,  \oracle'$, where   $\icinv{F_0, \ldots, F_k} $, and 
	$\forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh$. Towards this end, we propose the following loop invariant for the loop beginning in line~$3$:
	%
	%
	\begin{align*}
	%
	I \eeq& \forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh \eewedge  \left( I_1 \eevee I_2 \right),~\text{where} \\[0.4em]
	%
    I_1 \eeq& \qempty \eewedge \icinv{F_0,\ldots,F_k}  \\[0.4em]
    %
    I_2 \eeq&  \nqempty \eewedge \icinv{F_0,\ldots,F_{k-1}} \eewedge F_{k-1} \leq F_k \eewedge \bm{F_{k-1}} \leq F_k \\[0.4em]
    			& \quad \eewedge \forall (i,s,\delta) \in Q \colon \left( i <k \vee (i,s,\delta) = (k, \sinit, \lambda) \right) 
	\end{align*}
	%
	%
	We now verify that the loop invariant $I$ holds at the beginning of the loop (initialization) and that it is preserved by each iteration (consecution).
	Notice that $ \forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \lambda$ holds at all times since no input except for the oracle $\oracle$ is altered during execution.  \\ \\
	%
	\noindent
	\textbf{Initialization.} We show that $I_2$ holds at the beginning of the loop. $\icinv{F_0,\ldots,F_{k-1}}$ holds by assumption.
	                                 Moreover, after line $1$, the priority queue $Q = \left\{ (k, \sinit,\lambda) \right\}$ is non-empty and satisfies
	                                 	$ \forall (i,s,\delta) \in Q \colon \left( i <k \eevee (i,s,\delta) = (k, \sinit, \lambda) \right) $. \\ \\
	%
	%
	\noindent
	\textbf{Consecution.} Assume the loop invariant $I$ holds at the beginning of some iteration. Due to the guard of the loop,
	we additionally know that $Q$ is non-empty. Hence, we know that $I_1$ does not hold, but $I_2$ does. We show that
	$I$ is reestablished after this iteration. The procedure first pops an element $(i, s, \delta)$ with minimal $i$ from $Q$ (line $4$).
	We distinguish the following two cases:
	%
	%
	%\begin{alignat}{2}
	%
	%\textnormal{Case 1:} \quad & Q.\qpop~\textnormal{returns}~(k,\sinit,\delta)  %\notag \\[0.3em]
	%
	%
	%\textnormal{Case 2:} \quad & Q.\qpop~\textnormal{does not %return}~(k,\sinit,\delta)   \notag
	%
	%\end{alignat}
	%
	%
	%
	\begin{alignat}{2}
	%
	\textnormal{Case 1:} \quad & i=0 \notag \\[0.3em]
	%
	%
	\textnormal{Case 2:} \quad & i\neq 0   \notag
	%
	\end{alignat}
	%
	\emph{Case 1.} Since $i=0$, we immediately enter the if-branch beginning in line $7$.
	Since $\forall n \colon \bmnapp{n}{\zeroexp}{\sinit} \leq \thresh$, there is no $\ostates \subseteq S$ such that $\prevmdpmax{\smdp{\ostates}}{\bad} > \thresh$.
	Consequently, the call to $\checkrefutation$ in line $8$ yields $\refute = \false$ (Definition~\ref{def:spec_checkrefute}.\ref{def:spec_checkrefute_norefute}). After executing line $13$, we have $Q = \{(k, \sinit, \lambda)\}$, i.e., $Q$ is non-empty and $\forall (i,s,\delta) \in Q \colon \left( i <k \eevee (i,s,\delta) = (k, \sinit, \lambda) \right)$. Since the frames
	are not modified, we still have $ \icinv{F_0,\ldots,F_{k-1}}$ and $F_{k-1} \leq F_k \wedge \bm{F_{k-1}} \leq F_k$.
	Hence, $I_2$ holds and the loop invariant $I$ is reestablished. \\ \\
	%
	\noindent
	\emph{Case 2.} Since $i\neq 0$, we enter the else-branch beginning in line $15$.
	 There are now two further cases:
	%
	\begin{alignat}{2}
	%
	\textnormal{Case 2.1:} \quad & \exists a \in \acts{s} \colon \bma{a}{F_{i-1}}[s] \eeg \delta \notag \\[0.3em]
	%
	%
	\textnormal{Case 2.2:} \quad & \neg \exists a \in \acts{s} \colon \bma{a}{F_{i-1}}[s] \eeg \delta   \notag
	%
\end{alignat}
	%
	%
	\emph{Case 2.1.} We enter the if-branch
	beginning in line $16$. 
	%Let $\{s_1,\ldots,s_n\} = \succs (s)$.
	If the call to $\getprobs$ in line $17$ yields $\success = \true$ (Definition~\ref{def:spec_getprobs}.\ref{def:spec_getprobs_exists}), we enter the if-branch beginning in line $19$. Executing lines $19$ and $20$ does not violate $ \forall (i,s,\delta) \in Q \colon \left( i <k \eevee (i,s,\delta) = (k, \sinit, \lambda) \right)$
	since $0 < i \leq k$. Finally, the frames are not modified so that $I_2$ and thereby loop invariant $I$ holds.
	
	If the call to $\getprobs$ in line $17$ yields $\success = \false$, 
	the situation is analogous to case $1$. \\ \\
	%
	%
	\noindent
	\emph{Case 2.2.} We enter the else-branch beginning in line $30$. 
	Notice that 
	%
	\[
	\neg \exists a \in \acts{s} \colon \bma{a}{F_{i-1}}[s] \eeg \delta \quad \text{implies} \quad \bm{F_{i-1}}[s] \leq \delta~.
	\]
	%
	Hence, by Lemma~\ref{lem:ic3_inv_preserved_by_update},
	the update in line $30$ preserves the IC3-Invariants for $F_0,\ldots,F_i$. Notice that line $30$ can only make $F_i$ smaller. It is thus easy to see
	that $\icinv{F_0,\ldots,F_{k-1}}$ holds, as well. Now distinguish the cases $(i,s,\delta) = (k , \sinit, \lambda)$ and $(i,s,\delta) \neq (k , \sinit, \lambda)$. \\ \\
	%
	\noindent
	%
	\emph{The case $(i,s,\delta) = (k , \sinit, \lambda)$.} Our assumption $\forall (i,s,\delta) \in Q \colon \left( i <k \vee (i,s,\delta) = (k, \sinit, \lambda) \right)$ implies
	that $Q$ is empty now. After executing line $35$, we know that $F[\sinit] \leq \thresh$.
	%
	%
	We now verify that the IC3-Invariants hold for the frames $F_0, \ldots, F_k$. 
	Since they already hold for $F_0,\ldots,F_{k-1}$, we only need to check frame-safety of $F_k$, the chain-property for $F_k$ and $F_{k+1}$, and
	relative-inductiveness of $F_{k-1}$ and $F_k$. Frame-safety of $F_k$ is immediate since $F_k[\sinit] \leq \thresh$.
	Further, the update in line $35$ cannot lead to a violation of $F_{k-1} \leq F_k$. Finally, relative inductiveness of $F_{k-1}$ and $F_k$ still holds due to the check in line $15$.
	Overall, we have verified that $I_1$ holds and therefore $I$ is reestablished. \\ \\
	%
	\noindent
	%
	To complete our proof, now assume that the loop beginning in line $3$ terminates.
	Our loop invariant $I$ and the fact that $Q$ is empty (negation of the loop guard) implies 
	$\icinv{F_0,\ldots,F_k}$. Hence, $\strengthen$ returns $\false, F_0,\ldots,F_k,\oracle, \ostates$,
	where $F_0,\ldots,F_k$ satisfy the IC3-Invariants, which is what we had to show.	

%
%


==> strengthen-complete.tex <==
\sebastian{
Refer and explain algorithm}
\sebastian{precisely explain how progress states are build}
\input{algorithms/algorithm_strenghten}
